Omni-RGPT: Unifying Image and Video Region-level Understanding via Token Marks

We present Omni-RGPT, a multimodal large language model designed to facilitate region-level comprehension for both images and videos. To achieve consistent region representation across spatio-temporal dimensions, we introduce Token Mark, a set of tokens highlighting the target regions within the visual feature space. These tokens are directly embedded into spatial regions using region prompts (e.g., boxes or masks) and simultaneously incorporated into the text prompt to specify the target, establishing a direct connection between visual and text tokens. To further support robust video understanding without requiring tracklets, we introduce an auxiliary task that guides Token Mark by leveraging the consistency of the tokens, enabling stable region interpretation across the video. Additionally, we introduce a large-scale region-level video instruction dataset (RegVID-300k). Omni-RGPT achieves state-of-the-art results on image and video-based commonsense reasoning benchmarks while showing strong performance in captioning and referring expression comprehension tasks.

==> fig/data_vis.tex <==

\begin{figure*}[t!]\centering
\begin{minipage}{0.3\columnwidth}
 \vspace{0.8\columnwidth}
\begin{tcolorbox}[left=-0.2mm,top=-0.5mm,bottom=-0.2mm]
    \centering
    \footnotesize
    \begin{tabular}{p{\columnwidth} c}
\colorbox{maskpink}{[0]}: Cat & \\
\colorbox{maskorange}{[1]}: Cat & \\
\colorbox{maskblue}{[2]}: Hand 
    \end{tabular}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{1.6\columnwidth}
\footnotesize
\multirow{4}{*}{ 
  \begin{minipage}[b]{0.25\columnwidth}
    \includegraphics[width=\columnwidth]{fig/data_visualiation/fcd9cd4aec41_000008.jpg}
  \end{minipage}
  \begin{minipage}[b]{0.25\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/data_visualiation/fcd9cd4aec41_000024.jpg}
  \end{minipage}
  \begin{minipage}[b]{0.25\columnwidth}
    \includegraphics[width=\columnwidth]{fig/data_visualiation/fcd9cd4aec41_000059.jpg}
  \end{minipage}
  \begin{minipage}[b]{0.25\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/data_visualiation/fcd9cd4aec41_000119.jpg}
  \end{minipage}
}\end{minipage} \vspace{1mm}  \\  \hrulefill \begin{minipage}{2.0\columnwidth}\end{minipage}\\ 
\begin{minipage}{0.66\columnwidth}
\begin{tcolorbox}[title=Stage-I: Region-level Caption, left=-0.2mm] 
    \centering
      \footnotesize
    \begin{tabular}{p{\columnwidth} c}
{\color{\maskpink}{[0]}}: The cat is partially visible on a wooden bench, sitting upright and looking towards the camera. It is positioned near a white post that divides the sitting area. In the background, there are lush green trees and a paved path, ... (omitted, 60 words) & \\
\colorbox{maskorange}{[1]}: The cat is lying on a wooden bench, fully stretched out with its head resting on its front paws. The cat seems content,  ...(omitted, 57 words) & \\
\colorbox{maskblue}{[2]}: The person's hand is reaching out to pet the cat on the bench. Only the arm is visible, extending towards the cat and offering gentle strokes along the cat's back and head. ... (omitted, 67 words) & \\ 
%& \\
    \end{tabular}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
\centering
\begin{tcolorbox}[title=Stage-II: Hallucination Mitigation, left=-0.2mm] 
    \centering
      \footnotesize
    \begin{tabular}{p{\columnwidth} c}
\bf{Closed-Ended QAs for} \colorbox{maskpink}{[0]}: & \\
Q1: Is the cat partially visible on a wooden bench? Select from (A): Definitely Yes, (B): Possibly No, (C): Possibly No, (D): Definitely No, (E): Not sure. & \\
Q2: Is the cat sitting upright? Select from (A): Definitely Yes... & \\
% Q3: Is the cat looking towards the camera? Select from ... & \\
... & \\ 
\bf{Refined Caption for} \colorbox{maskpink}{[0]}: & \\
 The cat \erase{is partially visible on a wooden bench, sitting upright and looking towards the camera. It} is positioned near a white post that divides the sitting area. In the background, there are lush green trees and a paved path, .... (omitted)
    \end{tabular}
\end{tcolorbox}
\end{minipage}
\begin{minipage}{0.66\columnwidth}
\centering
\begin{tcolorbox}[title=Stage-III: Instruction Generation, left=-0.2mm] 
    \centering
      \footnotesize
    \begin{tabular}{p{\columnwidth} c}
\textcolor{nvgreen}{{\bf Type 1: region-level brief description}} & \\
{\bf USER}: Provide a short description of \colorbox{maskblue}{[2]}.  &\\
{\bf ASSISTANT}: A person's hand pets a cat on a bench, creating a calm park atmosphere. & \\
\textcolor{nvgreen}{{\bf Type 2: region-level detailed description}}& \\
 {\bf USER}: Provide a detailed account of the object located at \colorbox{maskorange}{[1]} in the video. & \\
 {\bf ASSISTANT}: The cat is lying on a wooden bench, fully stretched out with its head resting on its front paws....(omitted, 57 words) & \\
\textcolor{nvgreen}{{\bf Type 3: region-level conversation}}& \\
 {\bf USER}: What is the cat next to in \colorbox{maskpink}{[0]}? & \\
  {\bf ASSISTANT}: The cat is positioned near a white post that divides the sitting area. &
    \end{tabular}
\end{tcolorbox}
\end{minipage}
\caption{\textbf{Our instruction data curation pipeline.}}
    \label{fig:data_visualization}
\end{figure*}


==> tab/video-rec.tex <==
\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccc|c}
\toprule
 & RGPT~\cite{RGPT} & Groma~\cite{Groma} & LLaVA-OV~\cite{LLaVAOneVision}+SoM~\cite{SoM} & Elysium~\cite{Elysium} & Ours \\ \midrule
val  & - & - & - & - & 37.5 \\
test & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{\textbf{VideoREC on Vid-STG val and test set}.}
\label{tab:video-rec}
\end{table}
